Stop Overvaluing Multi-Agent Debate -- We Must Rethink Evaluation and Embrace Model Heterogeneity

Multi-agent debate (MAD) has gained significant attention as a promising line of research to improve the factual accuracy and reasoning capabilities of large language models (LLMs). Despite its conceptual appeal, current MAD research suffers from critical limitations in evaluation practices, including limited benchmark coverage, weak baseline comparisons, and inconsistent setups. This paper presents a systematic evaluation of 5 representative MAD methods across 9 benchmarks using 4 foundational models. Surprisingly, our findings reveal that MAD often fail to outperform simple single-agent baselines such as Chain-of-Thought and Self-Consistency, even when consuming significantly more inference-time computation. To advance MAD research, we further explore the role of model heterogeneity and find it as a universal antidote to consistently improve current MAD frameworks. Based on our findings, we argue that the field must stop overvaluing MAD in its current form; for true advancement, we must critically rethink evaluation paradigms and actively embrace model heterogeneity as a core design principle.

==> 1_intro.tex <==
% \section{Introduction}
% With the widespread application of Large Language Models (LLMs), extensive attention has been paid to developing more advanced LLMs. As a simple taxonomy of techniques contributing to stronger LLMs, training-time computing and test-time computing improve LLMs in two stages during their lifetime. We have recently observed an increasing interest in test-time computing, which did not receive equivalent attention compared to training-time methods. 

% In this paper, we revisit one of the test-time computing methods, named \textbf{multi-agent debate (MAD)}. Multi-agent LLM debate primarily focuses on combining multiple LLM agents to collaboratively receive, analyze, exchange, integrate, and output information. In a typical workflow of MAD, agents first receive the query and give a solution independently. Then agents debate with each other to determine the final solution. This approach leverages the reasoning capabilities of multiple LLMs without additional training. Society of Minds (SoM) \hf{footnote for clarification}is the first MAD framework incorporating a group of LLM agents simultaneously solving the question and discussing a final answer. Some following works such as Multi-Persona (MP), and Exchange of Thoughts (EoT) continued to improve the MAD framework by introducing new mechanisms, e.g., agent confidence levels, to help agents debate more efficiently.

% However, these previous explorations into MAD have certain limitations. For instance, the evaluation in these works is limited to specific tasks without a comprehensive evaluation of the generalization capability of the proposed MAD framework. Additionally, we observe a lack of holistic assessment of how different decision designs might impact performance, e.g., the number of incorporated agents or the depth of the debating process. Furthermore, previous work also lacked sufficient comparisons between MAD and other advanced inference-stage baselines.

% Considering these limitations, in this paper we try to take a further step toward the design decision of existing MAD methods. Specifically, we try to answer three research questions: \textbf{RQ1)} Can current MAD methods perform consistently better than single-agent inference methods? \textbf{RQ2)} How do different dimensions of design decisions impact the performances of MAD? \textbf{RQ3)} What could be the future directions of MAD? We hope that, by answering these research questions, we can shed light on the future development of MAD methods. 

% The remaining part of this paper is organized as follows. In the second section, we will review previous MAD methods and propose a general framework integrating these MAD methods. Following the background we will introduce how we design our experiments and show our empirical results. Finally, we analyze the pattern found from the outcome and discuss several future directions based on our observation.

% \begin{comment}
% \section{Introduction v2}
% An age-old saying, \emph{two heads are better than one}, encapsulates the enduring lesson that collaboration often triumphs over solitary effort. While traditionally rooted in human interactions, this principle has recently found applications in the field of large language models (LLMs).
% One emerging line of research, commonly referred to as multi-agent debate or discussion (MAD), explores the potential of engaging multiple LLM agents in structured communications. 
% By enabling these agents to iteratively debate or discuss, researchers have shown that, without any additional training, the resulting final outputs can surpass those of a single model. Thus, MAD, attracting growing interest, is recognized as a potential strategy for test-time (or inference-time) computation. 


% A typical MAD works as follows: given a question, multiple LLM agents independently generate initial answers in parallel; over several rounds, agents review other agents' answers and incorporate collective feedback to refine their answers; finally, the refined answers are aggregated to output the final answer. 
% To stimulate critical thinking and divergent feedback, agents are often prompted to role-play certain personas, such as [.....]. 
% Moreover, [...show in what ways (e.g., summarizing the answers?) these approaches vary...] 
% Since MAD somewhat mirrors how humans engage in group discussions, it is perhaps unsurprising that MAD can improve the performance of LLMs at test-time.


% However, critical questions remain--- 
% %However, despite its appeal---aligning naturally with the intuition that deliberative collective thinking can improve the outputs---questions remain regarding its performance and efficiency, particularly when compared to single-agent test-time computation strategies.
    
% \end{comment}

\section{Introduction}
An age-old saying, \emph{two heads are better than one}, encapsulates the enduring lesson that collaboration often triumphs over solitary effort. While traditionally rooted in human interactions, this principle has recently found applications in the field of large language models (LLMs)~\citep{chatgpt, instructgpt, vicuna, guanaco, chatglm}.
One emerging line of research, commonly referred to as multi-agent debate or discussion (MAD)~\cite{duimproving, yin2023exchange, liang2023encouraging, chen2023agentverse, chanchateval, wang2024rethinking, smit2023we}, explores the potential of engaging multiple LLM agents in structured communications. 
By enabling these agents to iteratively debate or discuss, researchers have shown that, without any additional training, the resulting final outputs can surpass those of a single model. Thus, MAD, attracting growing interest, is recognized as a potential strategy for test-time (or inference-time) computation. 

\begin{table*}[htb]
\caption{High-level comparison of MAD frameworks.}
\label{tab:mad_features}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|lllllll}
\hline
           & Role-Play & Answer Generation         & \#Agents   & \#Rounds       & Post-procesisng & Heterogeneous \\ \hline
SoM              & N/A       & Majority Voting & Adjustable & Fixed          & N/A             & No            \\
Multi-Persona                 & Fixed     & Judger          & Fixed      & Early-stopping & N/A             & Yes           \\
EoT              & Fixed     & Majority Voting & Adjustable & Early-stopping & Confidence      & No            \\
ChatEval           & Fixed     & Majority Voting                & Adjustable & Early-stopping & N/A             & Yes           \\
AgentVerse        & Dynamic   & Judger          & Adjustable & Early-stopping & N/A             & Yes           \\ \hline
\end{tabular}}
\end{table*}

A typical MAD works as follows: given a question, multiple LLM agents independently generate initial answers in parallel; over several rounds, agents review other agents' answers and incorporate collective feedback to refine their answers; finally, the refined answers are aggregated to form the final answer. 
Besides, agents are often prompted to role-play certain personas, as shown by existing research, to be effective in stimulating critical thinking and divergent feedback.
Moreover, some advanced MAD frameworks incorporate a summarizer agent to dynamically construct the final answer when simple majority voting fails, e.g., on coding tasks~\cite{chen2023agentverse}. 
Since MAD somewhat mirrors how humans engage in group discussions, it is perhaps unsurprising that MAD can improve the performance of LLMs at test time by utilizing more inference budgets and aggregating diverse information extracted from multiple agents.

Some recent works \cite{smit2023we, wang2024rethinking} have paid attention to the working mechanism of MAD frameworks, investigating how different agents can collaborate to improve model performance. However, despite the appealing intuition that deliberative collective thinking can integrate larger inference-time computation as well as diverse knowledge to improve the outputs, questions remain regarding its performance w.r.t. efficiency, particularly when compared to single-agent test-time computation strategies. Can MAD obtain a corresponding level of performance improvement with a reasonable extra test-time computational cost? Can MAD gain consistent performance improvements as computational costs increase (in other words, can a stable scaling law be observed)? Can MAD meet our expectations by effectively aggregating the knowledge of different agents to produce more refined answers?

In this paper, we take a systematic review of existing MAD frameworks, with a special focus on their performance and efficiency in comparison to widely used single-agent inference techniques, such as Chain-of-Thought (CoT) and Self-consistency (SC). Our evaluation of 5 typical MAD frameworks on 9 benchmarks led us to a surprising conclusion---\emph{current MAD frameworks fail to consistently outperform simple single-agent test-time computation strategies, even with more test-time computation}. We further explored the impact of various configurations on MAD performance, including the number of agents, the rounds of debate, and the foundation models used by the agents, in an effort to mitigate the negative effects of suboptimal hyperparameter settings on MAD performance. We did not observe MAD effectively leveraging extra test-time computation to improve reasoning outcomes. After these extensive evaluations, we concluded that current MAD frameworks may not be a good choice for enhancing agent performance at inference time. 

%Inspired by recent developments in LLM agent routing and combination
However, we found that previous MAD studies often overlooked the importance of model heterogeneity, instead only using a single foundation model for evaluation. Our empirical results show that by mixing the outputs of multiple different LLMs, MAD can achieve further performance gain, even surpassing the best model among all incorporated ones. Analysis indicates that the mixed MAD framework can effectively integrate the useful information generated by different base models, thereby enhancing overall reasoning ability. Mixed-MAD demonstrates that model heterogeneity will be an important future direction for the further development of MAD, considering we have shown that MAD is not an efficient test-time computing method. In summary, our contributions are as follows:

\begin{itemize}
    \item We take a systematic review of 5 MAD frameworks, with comprehensive evaluations on 9 benchmarks. Our empirical results showed that MAD cannot consistently outperform baselines even with a larger inference budget.

    \item We conduct an in-depth analysis of the scaling efficiency of MAD, and from the analysis, we find that MAD does not effectively utilize extra inference budget, indicating that MAD is not an optimal test-time computing method.

    \item From the perspective of model heterogeneity, we proposed Mixed-MAD. Mixed-MAD can consistently improve MAD's performance across different benchmarks. This phenomenon suggests that incorporating different foundation models into MAD is a promising future direction. Based on our findings, we also discuss feasible future development directions for MAD.
\end{itemize}


%However, despite its appeal---aligning naturally with the intuition that deliberative collective thinking can improve the outputs---questions remain regarding its performance and efficiency, particularly when compared to single-agent test-time computation strategies.





==> 1_intro_v2.tex <==
% \section{Introduction}
% With the widespread application of Large Language Models (LLMs), extensive attention has been paid to developing more advanced LLMs. As a simple taxonomy of techniques contributing to stronger LLMs, training-time computing and test-time computing improve LLMs in two stages during their lifetime. We have recently observed an increasing interest in test-time computing, which did not receive equivalent attention compared to training-time methods. 

% In this paper, we revisit one of the test-time computing methods, named \textbf{multi-agent debate (MAD)}. Multi-agent LLM debate primarily focuses on combining multiple LLM agents to collaboratively receive, analyze, exchange, integrate, and output information. In a typical workflow of MAD, agents first receive the query and give a solution independently. Then agents debate with each other to determine the final solution. This approach leverages the reasoning capabilities of multiple LLMs without additional training. Society of Minds (SoM) \hf{footnote for clarification}is the first MAD framework incorporating a group of LLM agents simultaneously solving the question and discussing a final answer. Some following works such as Multi-Persona (MP), and Exchange of Thoughts (EoT) continued to improve the MAD framework by introducing new mechanisms, e.g., agent confidence levels, to help agents debate more efficiently.

% However, these previous explorations into MAD have certain limitations. For instance, the evaluation in these works is limited to specific tasks without a comprehensive evaluation of the generalization capability of the proposed MAD framework. Additionally, we observe a lack of holistic assessment of how different decision designs might impact performance, e.g., the number of incorporated agents or the depth of the debating process. Furthermore, previous work also lacked sufficient comparisons between MAD and other advanced inference-stage baselines.

% Considering these limitations, in this paper we try to take a further step toward the design decision of existing MAD methods. Specifically, we try to answer three research questions: \textbf{RQ1)} Can current MAD methods perform consistently better than single-agent inference methods? \textbf{RQ2)} How do different dimensions of design decisions impact the performances of MAD? \textbf{RQ3)} What could be the future directions of MAD? We hope that, by answering these research questions, we can shed light on the future development of MAD methods. 

% The remaining part of this paper is organized as follows. In the second section, we will review previous MAD methods and propose a general framework integrating these MAD methods. Following the background we will introduce how we design our experiments and show our empirical results. Finally, we analyze the pattern found from the outcome and discuss several future directions based on our observation.

% \begin{comment}
% \section{Introduction v2}
% An age-old saying, \emph{two heads are better than one}, encapsulates the enduring lesson that collaboration often triumphs over solitary effort. While traditionally rooted in human interactions, this principle has recently found applications in the field of large language models (LLMs).
% One emerging line of research, commonly referred to as multi-agent debate or discussion (MAD), explores the potential of engaging multiple LLM agents in structured communications. 
% By enabling these agents to iteratively debate or discuss, researchers have shown that, without any additional training, the resulting final outputs can surpass those of a single model. Thus, MAD, attracting growing interest, is recognized as a potential strategy for test-time (or inference-time) computation. 


% A typical MAD works as follows: given a question, multiple LLM agents independently generate initial answers in parallel; over several rounds, agents review other agents' answers and incorporate collective feedback to refine their answers; finally, the refined answers are aggregated to output the final answer. 
% To stimulate critical thinking and divergent feedback, agents are often prompted to role-play certain personas, such as [.....]. 
% Moreover, [...show in what ways (e.g., summarizing the answers?) these approaches vary...] 
% Since MAD somewhat mirrors how humans engage in group discussions, it is perhaps unsurprising that MAD can improve the performance of LLMs at test-time.


% However, critical questions remain--- 
% %However, despite its appeal---aligning naturally with the intuition that deliberative collective thinking can improve the outputs---questions remain regarding its performance and efficiency, particularly when compared to single-agent test-time computation strategies.
    
% \end{comment}

\section{Introduction}
An age-old saying, \emph{two heads are better than one}, encapsulates the enduring lesson that collaboration often triumphs over solitary effort. While traditionally rooted in human interactions, this principle has recently found applications in the field of large language models (LLMs).
%~\citep{chatgpt, instructgpt, vicuna, guanaco, chatglm}.
An emerging line of research, commonly referred to as multi-agent debate or discussion (MAD)~\cite{duimproving, yin2023exchange, liang2023encouraging, chen2023agentverse, chanchateval, wang2024rethinking, smit2023we}, explores the potential of engaging multiple LLM agents in structured communications. 
By enabling these agents to iteratively debate or discuss, researchers have shown that, without any additional training, the resulting final outputs can surpass those of a single model. Thus, MAD, attracting growing interest, is recognized as a potential strategy for test-time (or inference-time) computation. 

\begin{table*}[htb]
\caption{High-level comparison of MAD frameworks.}
\label{tab:mad_features}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|lllllll}
\hline
           & Role-Play & Answer Generation         & \#Agents   & \#Rounds       & Post-procesisng & Heterogeneous \\ \hline
SoM              & N/A       & Majority Voting & Adjustable & Fixed          & N/A             & No            \\
Multi-Persona                 & Fixed     & Judger          & Fixed      & Early-stopping & N/A             & Yes           \\
EoT              & Fixed     & Majority Voting & Adjustable & Early-stopping & Confidence      & No            \\
ChatEval           & Fixed     & Majority Voting                & Adjustable & Early-stopping & N/A             & Yes           \\
AgentVerse        & Dynamic   & Judger          & Adjustable & Early-stopping & N/A             & Yes           \\ \hline
\end{tabular}}
\end{table*}

A typical MAD works as follows: given a question, multiple LLM agents independently generate initial answers in parallel; over several rounds, agents review other agents' answers and incorporate collective feedback to refine their answers; finally, the refined answers are aggregated to form the final answer. 
Besides, agents are often prompted to role-play certain personas, as shown by existing research, to be effective in stimulating critical thinking and divergent feedback.
Moreover, some advanced MAD frameworks incorporate a summarizer agent to dynamically construct the final answer when simple majority voting fails, e.g., on coding tasks~\cite{chen2023agentverse}. 
Since MAD somewhat mirrors how humans engage in group discussions, it is perhaps unsurprising that MAD can improve the performance of LLMs at test time by utilizing more inference budgets and aggregating diverse information extracted from multiple agents.

Some recent works \cite{smit2023we, wang2024rethinking} have paid attention to the working mechanism of MAD frameworks, investigating how different agents can collaborate to improve model performance. However, despite the appealing intuition that deliberative collective thinking can integrate larger inference-time computation as well as diverse knowledge to improve the outputs, questions remain regarding its performance w.r.t. efficiency, particularly when compared to single-agent test-time computation strategies. Can MAD obtain a corresponding level of performance improvement with a reasonable extra test-time computational cost? Can MAD gain consistent performance improvements as computational costs increase (in other words, can a stable scaling law be observed)? Can MAD meet our expectations by effectively aggregating the knowledge of different agents to produce more refined answers?

In this paper, we take a systematic review of existing MAD frameworks, with a special focus on their performance and efficiency in comparison to widely used single-agent inference techniques, such as Chain-of-Thought (CoT) and Self-consistency (SC). Our evaluation of 5 typical MAD frameworks on 9 benchmarks led us to a surprising conclusion---\emph{current MAD frameworks fail to consistently outperform simple single-agent test-time computation strategies, even with more test-time computation}. We further explored the impact of various configurations on MAD performance, including the number of agents, the rounds of debate, and the foundation models used by the agents, in an effort to mitigate the negative effects of suboptimal hyperparameter settings on MAD performance. We did not observe MAD effectively leveraging extra test-time computation to improve reasoning outcomes. After these extensive evaluations, we concluded that current MAD frameworks may not be a good choice for enhancing agent performance at inference time. 

This counter-intuitive observation naturally challenges our previous belief that more test-time computation through multi-agent debate can improve overall performance. We believe this outcome is due to the current MAD framework not effectively leveraging the differences between models for more efficient reasoning. This hinders MAD from integrating the strengths of different agents, leading it to degrade into repetitive single-agent reasoning. We hypothesize that introducing model heterogeneity into the MAD framework can help MAD integrate the knowledge of different models, enabling more effective collaborative reasoning. To validate this hypothesis, we propose a simple and general strategy called \textbf{Mixed-MAD}. Our empirical results show that Mixed-MAD, by mixing the outputs of multiple different LLMs, can achieve further performance gain, even surpassing the best model among all incorporated ones. Analysis indicates that Mixed-MAD can effectively integrate the useful information generated by different base models, thereby enhancing overall reasoning ability. Mixed-MAD demonstrates that model heterogeneity will be an important future direction for the further development of MAD, considering we have shown that MAD is not an efficient test-time computing method. Future work may focus more on flexibly merging the knowledge of different models through debate, integrating their strengths, and complementing each other's knowledge gaps. In summary, our contributions are as follows:

\begin{itemize}
    \item We take a systematic review of 5 MAD frameworks, with comprehensive evaluations on 9 benchmarks. Our empirical results showed that MAD cannot consistently outperform baselines even with a larger inference budget.

    \item We conduct an in-depth analysis of the scaling efficiency of MAD, and from the analysis, we find that MAD does not effectively utilize extra inference budget, indicating that MAD is not an optimal test-time computing method.

    \item From the perspective of model heterogeneity, we proposed Mixed-MAD. Mixed-MAD can consistently improve MAD's performance across different benchmarks. This phenomenon suggests that incorporating different foundation models into MAD is a promising future direction. Based on our findings, we also discuss feasible future development directions for MAD.
\end{itemize}


%However, despite its appeal---aligning naturally with the intuition that deliberative collective thinking can improve the outputs---questions remain regarding its performance and efficiency, particularly when compared to single-agent test-time computation strategies.





==> 1_intro_v3.tex <==
% The remaining part of this paper is organized as follows. In the second section, we will review previous MAD methods and propose a general framework integrating these MAD methods. Following the background we will introduce how we design our experiments and show our empirical results. Finally, we analyze the pattern found from the outcome and discuss several future directions based on our observation.

% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=\textwidth]{image/main_pie.pdf}
%     \caption{Performance comparison of MAD across 4 models and 9 benchmarks. Each pie chart represents the distribution of conditions where MAD outperforms or does not outperform CoT.}
%     \label{fig:main_pie}
% \end{figure*}

% \begin{figure}[htb]
%      \centering
%      \includegraphics[width=0.48\textwidth]{image/fig1_2.pdf}
%         \caption{Our evaluation is structured around three pivotal dimensions: performance, efficiency, and robustness.}
%         \label{fig:1}
% \end{figure} 
\section{Introduction}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{image/fig1_4.pdf}
    %\caption{Our evaluation is structured around three pivotal dimensions: performance, efficiency, and robustness.}
    \caption{The promotion and recognition of MAD research require a systematic and comprehensive evaluation, structured around three pivotal dimensions: performance, efficiency, and robustness. }
    \label{fig:1}
\end{figure}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{image/win_rate.pdf}
    \caption{Performance comparison of MAD across 4 LLMs and 9 benchmarks, covering 3 top-level categories: general knowledge, mathematical reasoning, and programming. Each bar represents the distribution of conditions where MAD is better/comparable/worse than CoT. We employ the ANOVA test to evaluate differences among group means, considering a $p$-value greater than 0.05 as an indicator that no significant differences---a tie---exist. 
    %For SoM, MP, EoT, and AGV, we follow the authors' open-source implementations. For CE, which is in lack of an official open-source implementation as of 2024/10, we carefully reproduce it based on implementation details provided in the paper~\citep{chanchateval}. 
    }
    \label{fig:main_pie}
\end{figure*}



%\textcolor{purple}{Everybody's business is nobody's business. vs. two heads are better than one}

The age-old saying, \emph{two heads are better than one}, encapsulates the enduring lesson that collaboration often triumphs over solitary effort.
Can this human wisdom be applied to enhance the capabilities of large language models (LLMs)?
An emerging line of research---commonly known as multi-agent debate or discussion (MAD)---suggests it can. 
Research has shown that after multiple LLM agents independently produce initial answers to a question, by having them engage in several rounds of discussing and reviewing answers from each other, they can improve the factual accuracy and reasoning quality of their final aggregated response~\citep{duimproving}. As such, LLM performance is enhanced at inference time, without the need for additional training, suggesting MAD as an inference-time solution to boosting LLM capabilities.
Thus, unsurprisingly, this line of research has garnered significant attention, with prestigious venues witnessing a surge in the number of publications~\citep{ yin2023exchange, liang2023encouraging, chen2023agentverse, chanchateval, wang2024rethinking, smit2023we}.



Although we, like the community, believe in the potential of MAD, we position that \emph{this field has thus far suffered from a glaring lack of sufficiently systematic and comprehensive evaluations.}
%~\citep{duimproving, liang2023encouraging, yin2023exchange, chen2023agentverse, chanchateval}.
The datasets used for evaluation are limited and have minimal overlap between different MAD methods. 
While some focus on mathematical reasoning~\citep{duimproving, yin2023exchange}, others may target machine translation~\citep{liang2023encouraging}, 
%open-ended dialogue generation~\citep{chanchateval}, 
or programming tasks~\citep{chen2023agentverse}.
In some cases, a newly proposed MAD method is evaluated on another new dataset introduced in the same paper, which has not been fully disclosed~\citep{chanchateval}.
Moreover, newly proposed methods are often compared solely against the very basic approach of directly prompting LLM to generate answers. This overlooks simple single-agent techniques, such as Chain-of-Thought~\citep{cot}, as well as more recent advancements in MAD.
In addition, while evaluations are frequently performed using only proprietary LLMs, the efficiency of MAD that trade-off token consumption and performance gains have rarely been considered, with only few exceptions~\citep{smit2023we}.
%with a single set of parameter configurations. 

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{image/fig1.png}
%     \caption{Our evaluation is structured around three pivotal dimensions: performance, efficiency, and robustness.}
%     \label{fig:1}
% \end{wrapfigure}


These current common practices of MAD evaluation can easily give rise to significant doubts about the reproducibility and generalizability of MAD methods, while also creating confusion about the status quo of MAD research. Specifically, do MAD methods genuinely outperform existing methods? To what extent do they outperform simpler single-agent baselines? Among them, what is the state of the art? Do these methods demonstrate robust performance across diverse conditions, or is their success a mere result of cherry-picking---critically dependent on specific dataset choices and parameter settings? Do they excel in both performance and efficiency?
%To put it simply, one might suspect ``\emph{results demonstrating the superiority of a newly proposed method are obtained by an experimental design favorable to that method} \citep{herrmann2024position}''---a concern that has plagued many areas of empirical ML.
Undoubtedly, as long as these questions remain unresolved, they will continue to hinder the recognition and promotion of MAD research, even eroding the trust in MAD research, just as they have plagued many other areas of empirical ML~\citep{herrmann2024position}.


To this end, in this paper, we critically evaluate 5 representative MAD methods across 9 widely adopted benchmarks, spanning various key high-level LLM capabilities: general knowledge, mathematical reasoning, and programming, with 4 different LLMs and various parameter configurations. As illustrated in Figure \ref{fig:1}, our evaluation is structured around three pivotal dimensions: performance, efficiency, and robustness.
Our first set of experiments, comparing these MAD methods to single-agent approaches, including Chain-of-Thought (CoT) and Self-consistency (SC)~\citep{wang2022self}, reveal an astonishing negative result---\emph{these MAD methods generally fail to outperform CoT}, despite CoT being much simpler.
As summarized in Figure 1, none of these MAD methods achieve a win rate higher than 20\% when compared to CoT across 36 scenarios (4 models $\times$ 9 benchmarks).
Further experiments varying the number of agents and debate rounds show that simply adjusting these hyperparameters can hardly reverse this negative outcome.
Moreover, the underperformance becomes even more pronounced when compared to SC, especially when using a comparable number of LLM calls or tokens.
All these results point to a crucial reality---\emph{existing MAD approaches are less effective than currently believed, even underperforming simple single-agent methods like CoT and SC}---an insight that would have remained elusive without a systematic and comprehensive evaluation.

%This suggests that even consuming more tokens, these methods cannot effectively leverage the extra inference budget, reinforcing their non-superiority compared to single-agent approaches.

While the above results seem discouraging, we emphasize that they do \emph{not} imply MAD research is a frustrating dead end. After all, countless examples have demonstrated the power of human collaboration. 
Then, we must ask ourselves: \emph{do current MAD methods truly emulate how people engage in productive discussion?}
A key factor enabling meaningful discussion is the diversity of knowledge and experience among individuals. While different LLMs trained on different data and paradigms may exhibit distinct strengths likewise, this crucial aspect remains largely unexplored in current MAD research---where, when multiple LLM agents are employed, they are typically instantiated from the same model.
We hypothesize that \emph{incorporating model heterogeneity is an effective solution to improving MAD}.
To allow for a broad validation on this hypothesis, we introduce a simple twist that can be incorporated into \emph{any} existing MAD methods: instead of relying on a single model, agents randomly select an LLM from a diverse set of candidate models at inference time to generate responses. 
Despite its simplicity, this twist proves to be broadly effective, leading to performance gains for \emph{all} MAD methods considered.
Beyond model heterogeneity, based on our analysis, we also propose multiple key research questions for future work: (i) \emph{How can MAD be calibrated to fully leverage model heterogeneity?} (ii) \emph{What kind of application scenarios better reflect the utility of MAD?} and (iii) \emph{How to enhance MAD frameworks with single-agent inference approaches?}
Note that we intentionally refrain from delving into well-calibrated technical solutions, such as designing a MAD framework explicitly optimized for leveraging model heterogeneity, as we believe that the development of solutions along the aforementioned directions holds significant promise and merits further exploration within the community.




==> 2_background.tex <==
\section{Background}
In this section, we briefly review the background of MAD methods, with a special focus on their unique mechanisms. We also present a systematic comparison between these MAD methods from several commonly shared dimensions. 

% Based on the information flow through agents, current MAD methods can be represented as a directed graph, where each node corresponds to invoking an LLM agent, and each edge denotes the transfer of outcomes between agents. Specifically, the action performed at each node is defined as follows:
% Based on the information flow through agents, current MAD methods can be represented as a directed graph, where each node corresponds to invoking an LLM agent, and each edge denotes the transfer of outcomes between agents. Specifically, the action performed at each node is defined as follows:

% \begin{equation}
%     a \sim F(G(q,x;h,\bm{\theta},\beta,p))
% \end{equation}
% \\
% where $h$ denotes the chat history of the agent, $\theta$ denotes parameters of the pre-trained base model, $\beta$ denotes inference hyper-parameters, $p$ denotes formatting prompts guiding the debate, $q$ denotes the input question, and $x$ denotes the answers from other agents (output from input nodes). $G$ represents invoking an LLM agent with specified configurations and $F$ denotes the post-processing of the agent's output. For instance, in EoT, the post-processing function $F$ assigns a confidence score to each agent's output, enabling other agents to assess whether the outcome was generated with high confidence. These dimensions are considered since they can be flexibly adjusted in different MAD frameworks and are enough to cover the main components of MAD. 

% The final response, $a$, is sampled from the conditional distribution $F(G(\circ; \circ))$. A digraph denoted as $G= (V,E)$ can describe the architecture of the MAD framework. A directed edge $e = (v_i, v_j) \in E$ will transmit an output $a_i$ from node $v_i$ to its subsequent neighbor $v_j$, which gives $a_i \in x_j$. If $(v_i, v_j)$ is the only incoming edge for $v_j$, then $x_j=\{a_i\}$. Additionally, the workflow of MAD frameworks can sometimes be conditional, depending on specific outputs from certain agents. For instance, in AgentVerse, the verifier’s output may determine whether the solver is invoked again to provide a refined solution.

Inspired by \textbf{The Society of Mind}, ~\citet{duimproving} presented the first LLM-based MAD framework. In this framework, multiple agents independently generate proposals and collaboratively engage in deliberation on their respective reasoning processes to reach a consensus on a unified response. The answers may be optionally summarized before being added to the history that is available to the agents in future rounds. To avoid misunderstanding, in the following part of this paper we refer to ~\citet{duimproving} as \textbf{SoM}.

\textbf{Multi-Persona (MP)} \cite{liang2023encouraging} leverages the role-playing capabilities of LLMs to encourage diverse thinking. In this approach, an affirmative agent(angel) and a negative agent(devil) present their answer to a judge agent, which ultimately determines the final solution.

While leveraging multi-persona role-playing, \textbf{ChatEval (CE)} \cite{chanchateval} explores communication strategies among agents through three frameworks, focusing on the impact of asynchronous responses and round-by-round summarization on agent performance.


\textbf{Exchange-of-Thought (EoT)} \cite{yin2023exchange} similarly emphasizes the study of communication strategies. It introduces four distinct communication paradigms and undertakes a comprehensive analysis of communication volume and information propagation speed. Additionally, it implements a confidence evaluation mechanism designed to reduce the adverse effects of erroneous reasoning processes.


\textbf{AgentVerse (AGV)} \cite{chen2023agentverse} is a meticulously designed and sophisticated multi-agent collaboration framework, distinct from conventional MAD frameworks. In AgentVerse, an agent will take the role of HR to hire experts to collaboratively draft the solution, allowing dynamic adjustment of group members based on current progress.


In Table \ref{tab:mad_features} (in Appendix \ref{appendix:mad_conf}) we compare these MAD frameworks from different dimensions of their implementation. As the first MAD framework, SoM simply aggregates information from agents without much processing. Following works 

==> 2_background_v2.tex <==
\section{Background}

MAD methods have garnered significant attention in recent years due to their potential to enhance the reasoning and decision-making capabilities of large language models (LLMs). These methods build on the idea of leveraging multiple interacting agents to collaboratively solve problems. In this section, we briefly review the background of MAD methods, with a special focus on their unique mechanisms. We also present a systematic comparison between these MAD methods from several commonly shared dimensions. 

At their core, MAD methods share several common principles. They typically involve multiple agents generating and evaluating responses, engaging in structured communication to refine their reasoning, and reaching a consensus through collaboration. This collaborative process utilizes more test-time inference budget than single-agent reasoning to improve the reasoning capability.

Despite these shared principles, different MAD methods exhibit varied considerations. 

\begin{itemize}
    \item Dynamic Adjustments: AgentVerse\cite{chen2023agentverse} dynamically assigns roles to agents to handle evolving problem contexts effectively. Such dynamic adjustment grants MAD more flexible capability to handle varied tasks.

    \item Consensus Mechanisms: Another key consideration is how consensus is derived. Beyond simple majority voting\cite{duimproving}, some MAD frameworks\cite{liang2023encouraging} adopted a judger agent to formulate the final answer.

    \item Agent Heterogeneity: Agents equivalently solve the task in basic MAD designs\cite{yin2023exchange, duimproving}. However, by introducing diverse roles such as judger, reviewer, or verifier, ChatEval\cite{chanchateval} and AgentVerse\cite{chen2023agentverse} make it possible for agents to view the problem through diverse aspects. 
\end{itemize}

In summary, MAD research explores a range of strategies for fostering collaboration among agents while addressing unique challenges such as communication efficiency and adaptability. These innovations collectively highlight the growing importance of MAD frameworks in advancing LLM capabilities. 

However, we note that current MAD research has certain shortcomings in evaluation. Specifically, SoM, AgentVerse, and ChatEval were not compared against CoT on these widely used benchmarks. MP was evaluated against CoT only on a handcrafted dataset named Counter-Intuitive Arithmetic Reasoning (CIAR). EoT was compared to CoT on GSM8k only, in which EoT was shown to be slightly better than CoT. Recently, \cite{smit2023we} analyzed the MAD method and found that the frequency of agents agreeing with each other in MAD has a direct impact on overall performance. However, \cite{smit2023we} did not consider MAD as a test-time computation method and did not reach a consistent conclusion regarding the performance comparison between MAD and single-agent inference methods. In contrast, this paper systematically and comprehensively evaluates the performance of representative MAD frameworks across different scenarios and compares them with single-agent methods. Specifically, the testing and analysis in this paper focus on the perspective of test-time computation, thereby verifying whether MAD frameworks are suitable as test-time computation methods.

==> 2_background_v3.tex <==
\section{Related Works}
In this section, we first briefly review the background of the 5 representative MAD methods, with a special focus on their unique mechanisms. Next, we introduce some recent works that also review MAD methods and explain how our work differs from theirs.

\subsection{MAD frameworks}

~\citet{duimproving} presented the first LLM-based MAD framework. In this framework, multiple agents independently generate proposals and collaboratively engage in deliberation on their respective reasoning processes to reach a consensus on a unified response. To avoid misunderstanding, in the following part of this paper we refer to ~\citet{duimproving} as \textbf{SoM}.

\textbf{Multi-Persona (MP)} \cite{liang2023encouraging} leverages the role-playing capabilities of LLMs to encourage diverse thinking. In this approach, an affirmative agent(angel) and a negative agent(devil) present their answer to a judge agent, which ultimately determines the final solution.

While leveraging multi-persona role-playing, \textbf{ChatEval (CE)} \cite{chanchateval} explores communication strategies among agents through three frameworks, focusing on the impact of asynchronous responses and round-by-round summarization on agent performance.


\textbf{Exchange-of-Thought (EoT)} \cite{yin2023exchange} similarly emphasizes the study of communication strategies. It introduces four distinct communication paradigms and undertakes a comprehensive analysis of communication volume and information propagation speed. Additionally, it implements a confidence evaluation mechanism designed to reduce the adverse effects of erroneous reasoning processes.


\textbf{AgentVerse (AGV)} \cite{chen2023agentverse} is a meticulously designed and sophisticated multi-agent collaboration framework, distinct from conventional MAD frameworks. In AgentVerse, an agent will take the role of HR to hire experts to collaboratively draft the solution, allowing dynamic adjustment of group members based on current progress.

\textbf{FORD}~\cite{xiong-FORD} mitigates the inconsistency as the debate processes, and introduces a judge agent to summarize the debate results.

\textbf{ReConcile}~\cite{chen2024reconcile} adopts confidence-weighted voting to help consensus seeking. 

\textbf{COMM}~\cite{chen2024comm} encourage diverse thinking in the debate by assigning different reasoning paths to agents with different roles.

\textbf{IoA}~\cite{chen2024IoA} organizes agents in a network structure, splitting agents into blocks for better collaboration. 

In \cite{li2024Sparse}, agents communicate through a sparse topological structure. This sparse configuration enhances the depth of collaborative reasoning, enabling more complex inference.

\citet{qian2024scaling} investigated the scaling effects of MAD systems. By constructing various topological structures, the authors found that MAD systems can achieve consistent performance improvements as more agents participate in the reasoning process.

\citet{pham2023let} introduced a novel approach where agents interact using token embeddings instead of natural language. Compared to natural language, token embeddings can convey additional information, such as an agent’s confidence in specific key information.

\subsection{Recent works reviewing MAD}

\citet{smit2023we} evaluated several MAD methods, particularly their performance on medical benchmarks. The authors observed that the level of agreement among agents within MAD frameworks is a critical factor influencing performance. When agents are more inclined to agree with one another, the overall performance improves. However, this study does not comprehensively compare these MAD methods with single-agent inference techniques, leaving the scalability of MAD inconclusive. 

\citet{khan2024debating} analyzed the performance of MAD systems from the perspective of persuasiveness. Instead of testing existing MAD methods, the study examined the impact of model persuasiveness on the overall performance of the MAD framework in a generic scenario involving two debater agents and one judger agent. The authors found that more persuasive models (often stronger models) could enhance the overall performance of the MAD system, even when the judger was a weaker model. While this study delves into the underlying mechanisms of MAD, its focus does not align with the primary goals of our research.

\citet{wang2024rethinking} compared single-agent methods with MAD methods and found that when a single agent is provided with sufficiently detailed problem descriptions and demonstrations to assist its reasoning, single-agent inference can achieve approximate performance to MAD methods. However, this study evaluated only three datasets rather than a comprehensive set of commonly used ones. Furthermore, the single-agent inference method used for comparison was not a widely adopted approach, limiting the generalizability of the findings.

\citet{zhang2023exploring} explores the behavioral logic of MAD from the perspective of social psychology. By combining agents with different individual traits (e.g., stubbornness or conformity ) within an experimental framework, the authors found that certain combinations of personality can enhance the overall performance of the MAD system.


In summary, while some recent works established an initial review of existing MAD frameworks, they have certain limitations that prohibit us from understanding the gap between MAD and other single-agent inference methods. Furthermore, these works lack special attention to MAD's scalability performance, which is a significant limitation considering the community-wide expectation of MAD to be an efficient way to utilize aggregated inference strength. Therefore, it is necessary to establish a more comprehensive evaluation of MAD frameworks, with a special focus on their scaling behavior.

